Beyond Arrow's Impossibility: Fairness as an Emergent Property of Multi-Agent Collaboration

Fairness in language models is typically studied as a property of a single, centrally optimized model. As large language models become increasingly agentic, we propose that fairness emerges through interaction and exchange. We study this via a controlled hospital triage framework in which two agents negotiate over three structured debate rounds. One agent is aligned to a specific ethical framework via retrieval-augmented generation (RAG), while the other is either unaligned or adversarially prompted to favor demographic groups over clinical need. We find that alignment systematically shapes negotiation strategies and allocation patterns, and that neither agent's allocation is ethically adequate in isolation, yet their joint final allocation can satisfy fairness criteria that neither would have reached alone. Aligned agents partially moderate bias through contestation rather than override, acting as corrective patches that restore access for marginalized groups without fully converting a biased counterpart. We further observe that even explicitly aligned agents exhibit intrinsic biases toward certain frameworks, consistent with known left-leaning tendencies in LLMs. We connect these limits to Arrow's Impossibility Theorem: no aggregation mechanism can simultaneously satisfy all desiderata of collective rationality, and multi-agent deliberation navigates rather than resolves this constraint. Our results reposition fairness as an emergent, procedural property of decentralized agent interaction, and the system rather than the individual agent as the appropriate unit of evaluation.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> oldcom.tex <==


\begin{comment}
    
\begin{abstract}
Fairness in artificial intelligence is typically studied as a property of a single, centrally optimized model: formally, ensuring that outcomes are distributed equitably across demographic groups. As large language models become increasingly agentic and are deployed in multi-agent settings, fairness instead emerges through interaction and exchange. We study fairness through the problem of resource allocation in a multi-agent debate framework, where two agents negotiate allocations under differing ethical and ideological conditions. One agent is aligned to a specific ideology using retrieval-augmented generation, while the other remains unaligned or is adversarially biased. Across multiple ethical alignments, we find that alignment systematically structures negotiation strategies and allocation patterns, but does not guarantee convergence or full correction of biased proposals. In adversarial settings, aligned agents often function as partial moderators, restoring access for marginalized groups and constraining extreme demographic exclusion. However, persistent bias in interacting agents frequently survives debate, even under alignment constraints. These dynamics mirror the limits formalized by\textit{ Arrow’s Impossibility Theorem: no aggregation mechanism over individual preferences can simultaneously satisfy fairness, consistency, and non-dictatorship}. Analogously, in multi-agent LLM systems, ethical alignment cannot universally reconcile competing values through interaction alone. Our results reposition fairness as an emergent, procedural property of decentralized agent interaction rather than a static design constraint of individual models. Alignment improves damage containment and behavioral stability, but fairness ultimately depends on the dynamics of negotiation and preference aggregation among agents.\end{abstract}

\section{Introduction}
\label{submission}
Agentic Language Models are becoming a common technology for solving higher-level tasks such as planning, coordination, and BLBAL. These systems are increasingly positioned to influence decisions that carry material consequences \cite{plaat2025multi}. 
% As Large Language Models (LLMs) are getting more and more integrated into day-to-day life and agentic AI is becoming more common for higher-level tasks such as planning, coordination, and policy recommendation, these systems are increasingly positioned to influence decisions that carry material consequences \cite{plaat2025multi}. 
From healthcare triage \cite{mantena2025fine, ahmed2026large} and public service allocation to hiring pipelines and financial approvals \cite{sukharevsky2025seizing}, language models are no longer confined to generating text but are actively shaping resource flows and institutional outcomes. These high impact domains of application question fairness of resource allocation, as language models were shown to be highly skewed in their decision  \ref{}. Furthermore, in many of these contexts, decisions do not always arise from a model acting alone, but from networks of interacting agents that deliberate, exchange justifications, and revise proposals over time. As a result, the fairness of outcomes depends not only on how individual models are aligned, but on how their alignment behaves under negotiation, disagreement, and strategic pressure. By alignement, we ...  As we transition into multi-agentic AI, these systems do not merely output fixed values; fairness ceases to be a static property of alignment and becomes a dynamic property of interaction. 
% In practice, resource allocation is rarely the result of a single, static optimization. Instead, it is an emergent outcome of negotiation, contestation, and compromise among multiple actors-each operating with partial information, strategic incentives, and divergent normative commitments.they deliberate, negotiate, critique, and revise decisions through natural language. Under these conditions,
 
Sociologically, this process mirrors the \textbf{Negotiated Order Theory} \cite{strauss1978negotiations}, which posits that institutional outcomes, such as clinical triage, are not dictated by rigid rulebooks but are continuously reconstituted through the persuasive interactions of actors with competing professional priorities. In a multi-agent framework, agents representing different ideologies act as \textbf{Street-Level Bureaucrats} \cite{lipsky1980street}, utilizing their discretionary power to interpret needs. The final allocation is thus shaped by a cycle of persuasion and repeated correction, a process that risks being reduced to mere \textbf{Commensuration} \cite{espeland1998commensuration} where the complexities of human vulnerability are simplified into competitive metrics.

However, the shift toward a deliberative multi-agent system introduces a fundamental mathematical bottleneck described by \textbf{Arrow’s Impossibility Theorem} \cite{arrow1951social}. When agents attempt to aggregate diverse normative commitments into a single collective decision, Arrow’s theorem proves that no social choice mechanism can simultaneously satisfy non-dictatorship, Pareto efficiency, and the \textbf{Independence Irrelevant Alternatives}. In a multi-agent clinical setting, this implies that the negotiation process will inevitably encounter irrational cycles or be forced to default to a dictatorship of one logic-often the one most aligned with systemic clinical urgency-unless the deliberative framework is structurally protected. To utilize the stalemate predicted by Arrow, the interaction must move toward the principles of Communicative Action \cite{habermas1981theory}, where fairness is found not in the initial alignment of models but in the Procedural Justice of the debate. By treating fairness as a dynamic interaction, we acknowledge that we can emerge fairness out of interactional abilities aligning to a more ideological and social idea of what fairness truly is.

To our knowledge, most alignment research evaluates language models in isolation: a single model is prompted with a task, and its output is assessed against predefined normative or ethical criteria \cite{}. Within this paradigm, techniques such as retrieval-augmented generation (RAG), constitutional training, and preference optimization are used to encode value constraints directly into model behavior, implicitly treating fairness and alignment as intrinsic properties of an individual decision-making agent \citep{askell2021constitutional, ouyang2022training, lewis2020retrieval}. This evaluation setting assumes that once a model is aligned, its outputs will reliably reflect the intended ethical standards at deployment time.

However, this assumption weakens in multi-agent settings, where aligned models interact with other agents that may be unaligned, strategically self-interested, or explicitly biased. In such environments, outcomes are no longer determined solely by the internal objective of any single agent, but by the procedural dynamics of negotiation, persuasion, and conflict resolution among agents \citep{park2023generative, bianchi2024agent, silver2024testtime}. Even when one agent is ethically aligned, interaction can reintroduce bias through asymmetric persuasion, strategic framing, or persistent adversarial proposals, leading to collective outcomes that diverge from the aligned agent’s normative intent.

In this work, we study fairness as an emergent property of multi-agent LLM negotiation. We construct a controlled resource allocation environment with hard feasibility constraints and structured three-round debates. \textcolor{sage}{Agent A} is explicitly aligned to a normative ethical framework via RAG. \textcolor{blue}{Agent B} operates either without alignment or under adversarial prompts that induce demographically biased decision-making. The agents must propose allocation vectors, critique each other’s reasoning, and attempt to produce a joint final recommendation.

Our investigation centers on three questions.
\begin{itemize}
    \item \textit{First, How does ethical alignment of an individual large language model agent influence negotiation behavior and resource allocation outcomes in a multi-agent debate setting?s?}
\item \textit{Second, To what extent can an ethically aligned agent mitigate or correct biased allocation proposals when interacting with unaligned or adversarially biased agents?}
\item \textit{Third, How do interaction protocols and agentic exchange shape fairness outcomes in decentralized multi-agent LLM systems, beyond what is implied by the alignment properties of individual agents?}

\end{itemize}

Across multiple ethical frameworks and experimental settings, we find that alignment consistently structures behavior and stabilizes proposal trajectories. Aligned agents maintain coherent normative commitments across rounds and resist extreme demographic exclusion. However, alignment does not ensure convergence. In adversarial settings, biased proposals can persist despite repeated critique. The dominant effect of alignment is not full normative correction, but damage containment: aligned agents reduce the severity of unfair allocations without necessarily eliminating bias altogether.

These findings suggest that fairness in multi-agent LLM systems is procedural rather than purely objective. It arises from negotiation dynamics among agents with competing incentives and varying degrees of alignment. Ethical alignment remains valuable, but its benefits are interaction-dependent. As LLMs increasingly operate in decentralized and collaborative settings, understanding fairness as an emergent interactional property becomes essential for evaluating and governing agentic AI systems.
\section{Related Works}
Fair resource allocation has traditionally been studied as a property of centralized decision rules. Normative frameworks such as utilitarianism, egalitarianism, Rawlsian justice, and the capabilities approach provide competing prescriptions for distributing scarce goods \citep{rawls1971theory,sen1979equality,sen2009idea,dworkin1981equality}. These perspectives have been formalized in social choice theory through welfare aggregation principles such as Pareto efficiency, leximin ordering, and envy-freeness \citep{arrow1951social,moulin2003fair}. In machine learning, fairness has similarly been encoded as a constraint or optimization objective applied to a single predictive model \citep{dwork2012fairness,zafar2017fairness,corbett2018measure,chouldechova2020snapshot}. Within resource allocation and operations research, fairness is embedded directly into constrained optimization formulations \citep{bertsimas2011fairness}.

Across these traditions, fairness is typically treated as a property of a single model or centralized mechanism.
recent literature has shifted toward viewing fairness as a dynamic property of Multi-Agent Systems (MAS). Empirical studies by \cite{mouri2026evaluating, madigan2025emergent} have documented how interaction can surface or amplify biases. These range from discriminatory pricing in buyer-seller games to emergent bias in financial decision-making that is not traceable to individual components. Complementing this, \cite{binkyte2025interactional} introduced Interactional Fairness, framing fairness as a behavioral signal rooted in communicative respect and justification quality rather than mere resource distribution.

Our work diverges from these empirical foundations by grounding the limits of MAS fairness in Social Choice Theory. While prior work focuses on the observation of bias, we leverage Arrow’s Impossibility Theorem to argue that the failure to reach a perfectly fair consensus is an inherent structural constraint of decentralized preference aggregation. Furthermore, moving beyond fixed personas, we utilize Retrieval-Augmented Generation (RAG) to dynamically inject explicit ethical ideologies such as Utilitarianism or Egalitarianism at inference time. This allows us to test how specific philosophical frameworks function as partial moderators in adversarial settings, providing a robust theoretical and methodological account of how alignment can constrain, if not entirely eliminate, emergent systemic bias.

Recent research extends fairness considerations to multi-agent and dynamic environments. Temporal analyses show that fairness violations may accumulate across repeated decisions even when individual allocations appear locally reasonable \citep{kumar2023temporal}. In multi-agent reinforcement learning, fairness objectives have been incorporated through reward shaping, incentive mechanisms, and welfare-based optimization \citep{vengerov2007dynamic,kumar2023scarce,kumar2025decaf,kumar2025giff}.

These approaches model fairness as a numerical objective within decentralized learning systems. However, fairness remains encoded in reward signals or centralized evaluators rather than negotiated through language-mediated deliberation. Agents optimize scalar objectives, but they do not defend, revise, or justify normative commitments through structured debate. Our work departs from reward-based formulations by examining fairness as a procedural outcome of interaction among autonomous language agents.

Large language models have recently been extended into interactive, multi-agent systems capable of planning, coordination, and structured debate \citep{park2023generative,li2023camel,wu2023autogen}. Debate-based methods demonstrate that adversarial critique can improve reasoning quality and factual robustness \citep{du2023debate,irving2018debate,shah2018debate}.

While these works show that interaction shapes epistemic outcomes, they do not examine fairness as a property of agent interaction. The focus is typically on correctness, planning efficiency, or reasoning improvement rather than normative allocation under scarcity. Our debate protocol builds on this literature but shifts the focus from factual correctness to ethical resource allocation, enabling analysis of how normative commitments evolve under negotiation.

Several studies evaluate moral reasoning and ethical alignment in LLMs across competing normative frameworks \citep{hendrycks2021ethics,sorensen2022ethical}. Alignment techniques such as constitutional prompting and high-level principle conditioning aim to guide model behavior without task-specific supervision \citep{askell2022constitutional,bai2022training}. However, these approaches largely assess alignment in single-model settings. The robustness of alignment under decentralized interaction particularly when paired with unaligned or adversarial agents remains underexplored.

Our work addresses this gap by studying whether ethical alignment guarantees convergence toward fair outcomes or instead functions as a moderating mechanism that limits harm without eliminating bias. Retrieval-augmented generation (RAG) has become a standard technique for grounding LLM outputs in external knowledge sources \citep{lewis2020rag,izacard2021fid}. While RAG improves controllability and factual grounding, recent work demonstrates that retrieval pipelines are vulnerable to poisoning and fairness-targeted manipulation \citep{zhang2025ragpoison,bagwe2025ragunfair}.

In allocation contexts, retrieved evidence can shape both the justification and perceived legitimacy of decisions. We extend this line of inquiry by analyzing how retrieval-grounded alignment behaves in adversarial multi-agent settings, and whether it can withstand biased negotiation pressure. Prior work has examined fairness objectives, decentralized allocation mechanisms, multi-agent LLM debate, and alignment techniques largely in isolation. What remains underexplored is how ethical alignment performs under decentralized, adversarial interaction.

